Privacy Policy Enforcement Guardrails for Data-Sensitive Retrieval-Augmented Generation

Standard PII filters often miss contextual data leakage in RAG systems, such as non-regulated attribute clusters that collectively identify individuals. We introduce a Privacy Policy Enforcement (PPE) framework using dual one-class density estimators with fused text embeddings and a calibrated abstain region for out-of-distribution inputs. Using an axis-stratified, multi-LLM synthetic data pipeline across medicine, finance, and law, we found that traditional Gaussian Mixture baselines fail on borderline-safe stress tests by focusing on linguistic register rather than content. Our proposed T3+OCSVM detector, trained on safe and borderline-safe data, achieves a borderline AUROC of 0.93+ while reducing false positives by 44-55 percentage points and maintaining millisecond latency. Compared to supervised MLP classifiers or 14B-parameter LLM judges, our framework offers superior operational suitability, as the former suffers from high abstention rates and the latter from latency and calibration issues. This methodology provides a robust stress-testing standard for any synthetic-data-trained classifier.

==> figures/Case-style_Confound.tex <==
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=2 by 1, horizontal sep=1.2cm},
  width=0.45\columnwidth, height=4.5cm,
  ybar, bar width=12pt,
  ylabel={AUROC},
  symbolic x coords={Medical, Finance, Law},
  xtick=data,
  ymin=0.5, ymax=1.0,
  nodes near coords, nodes near coords style={font=\tiny},
]
\nextgroupplot[title={(a) GMM (Naive)}]
  \addplot coordinates {(Medical, 0.99) (Finance, 0.98) (Law, 0.94)};
\nextgroupplot[title={(b) Stress Test}]
  \addplot[fill=red!30] coordinates {(Medical, 0.72) (Finance, 0.78) (Law, 0.75)};
\end{groupplot}
\end{tikzpicture}%
}
\caption{The case-style confound. (a) High within-distribution AUROC masks a significant performance drop (b) when evaluated against the borderline-safe stress test.}
\label{fig:confound}
\end{figure}

==> figures/Data_Pipeline.tex <==
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[
  font=\small,
  >=Stealth,
  node/.style={draw, minimum width=20mm, minimum height=8mm, align=center},
  seed/.style={node, fill=blue!5},
  proc/.style={node, fill=green!5},
  pool/.style={node, fill=orange!5},
  out/.style={node, fill=red!5},
]
  \node[seed] (s) {Seed corpora\\(Med/Fin/Law)};
  \node[proc, below=of s] (ax) {Axis sampler\\(QI $\times$ Frame $\times$ Style)};
  \node[pool, below=of ax] (llm) {LLM pool\\(Qwen, Mistral, Phi)};
  \node[out, below=of llm] (data) {Synthetic corpus\\(Safe / Unsafe / Borderline)};

  \draw[->] (s) -- (ax);
  \draw[->] (ax) -- (llm);
  \draw[->] (llm) -- (data);
\end{tikzpicture}%
}
\caption{Synthetic data generation pipeline. The same axis-stratified multi-LLM pipeline is instantiated three times across medical, finance, and law domains.}
\label{fig:pipeline}
\end{figure}

==> figures/System_Overview.tex <==
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  font=\small,
  >=Stealth,
  node distance=10mm and 14mm,
  box/.style={draw, rounded corners=2pt, minimum height=10mm,
              minimum width=22mm, align=center, inner sep=3pt},
  retr/.style={box, fill=blue!8},
  llm/.style={box, fill=orange!10},
  l1/.style={box, fill=green!10},
  l2/.style={box, fill=red!12, minimum width=30mm, very thick},
  outp/.style={box, fill=gray!10, minimum width=22mm},
]
  \node[box, fill=gray!5] (q)  {User\\query};
  \node[retr, right=of q]  (r)  {Retriever};
  \node[llm, right=of r]   (g)  {LLM\\generator};
  \node[l1, right=of g]    (l1) {Layer-1\\regex / NER};
  \node[l2, right=of l1]   (l2) {Layer-2\\dual one-class OOD\\(this work)};
  
  \node[outp, right=of l2, yshift=6mm]  (pass) {Safe pass};
  \node[outp, right=of l2]              (flag) {Flag /\\sanitize};
  \node[outp, right=of l2, yshift=-6mm] (abs)  {Abstain};

  \draw[->] (q)  -- (r);
  \draw[->] (r)  -- (g);
  \draw[->] (g)  -- (l1);
  \draw[->] (l1) -- (l2);
  
  \draw[->] (l2.east) -- (pass.west) node[midway, above, font=\tiny] {$\delta < \tau$};
  \draw[->] (l2.east) -- (flag.west) node[midway, right, xshift=2mm, font=\tiny] {$\delta > \tau$};
  \draw[->] (l2.east) -- (abs.west)  node[midway, below, font=\tiny] {both-OOD};

  \node[draw, dashed, gray, fit=(l2), inner sep=8pt, label={[gray]above:PPE Framework}] {};
\end{tikzpicture}%
}
\caption{Layered privacy enforcement for RAG. Layer-1 catches direct identifiers. Layer-2, the focus of this work, uses a dual one-class density estimator to detect contextual privacy leakage.}
\label{fig:system_overview}
\end{figure*}

==> figures/figures_all.tex <==
% =============================================================================
% TikZ figures for the merged paper.
% Required libraries (add to main.tex preamble):
%   \usepackage{tikz}
%   \usetikzlibrary{arrows.meta, positioning, shapes.geometric, fit,
%                   backgrounds, calc}
%   \usepackage{pgfplots}
%   \pgfplotsset{compat=1.18}
% =============================================================================

% -----------------------------------------------------------------------------
% FIGURE 1 — System overview (§4)
% Shows where Layer-2 detection sits in a deployed RAG pipeline.
% -----------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  font=\small,
  >=Stealth,
  node distance=10mm and 14mm,
  box/.style={draw, rounded corners=2pt, minimum height=10mm,
              minimum width=22mm, align=center, inner sep=3pt},
  retr/.style={box, fill=blue!8},
  llm/.style={box, fill=orange!10},
  l1/.style={box, fill=green!10},
  l2/.style={box, fill=red!12, minimum width=30mm, very thick},
  outp/.style={box, fill=gray!10, minimum width=22mm},
]
  \node[box, fill=gray!5] (q)  {User\\query};
  \node[retr, right=of q]  (r)  {Retriever};
  \node[llm,  right=of r]  (g)  {LLM\\generator};
  \node[l1,   right=of g]  (l1) {\textbf{Layer-1}\\regex / NER};
  \node[l2,   right=of l1] (l2) {\textbf{Layer-2}\\dual one-class OOD\\(this work)};

  % Three outputs, vertically stacked to the right of l2 with clean spacing
  \node[outp, fill=green!15, right=18mm of l2, yshift=12mm] (ok)   {Safe pass};
  \node[outp, fill=red!18,   right=18mm of l2]              (flag) {Flag /\\sanitize};
  \node[outp, fill=yellow!25, right=18mm of l2, yshift=-12mm] (abst) {Abstain /\\human review};

  \draw[->] (q)  -- (r);
  \draw[->] (r)  -- (g);
  \draw[->] (g)  -- (l1);
  \draw[->] (l1) -- (l2);
  \draw[->] (l2.east) -- (ok.west)   node[midway, above, font=\scriptsize, sloped]{$\delta < \tau$};
  \draw[->] (l2.east) -- (flag.west) node[midway, above, font=\scriptsize]{$\delta > \tau$};
  \draw[->] (l2.east) -- (abst.west) node[midway, below, font=\scriptsize, sloped]{both-OOD};
\end{tikzpicture}%
}
\caption{Layered privacy enforcement for RAG. Layer-1 regex/NER catches
direct identifiers (SSN, MRN, e-mail, named individuals). \textbf{Layer-2},
the contribution of this work, is a dual one-class density estimator
over the answer text that detects \emph{contextual} privacy leakage ---
quasi-identifier clusters, referential client voice, and indirect-QI
paraphrases that pass Layer-1. Outputs are routed to safe-pass, flag,
or abstain based on the discriminator score~$\delta$ and an explicit
both-OOD abstain region (\S\ref{sec:disc:bothood}).}
\label{fig:system}
\end{figure*}

% -----------------------------------------------------------------------------
% FIGURE 2 — Synthetic data generation pipeline (§5)
% Three domains share the same generator structure.
% -----------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  font=\small,
  >=Stealth,
  node distance=8mm and 16mm,
  % corpus: rectangle with double border (data-store metaphor)
  corpus/.style={draw, double, double distance=1pt, rounded corners=2pt,
                 fill=blue!8, align=center, inner sep=4pt,
                 minimum width=24mm, font=\footnotesize},
  % sampler: parallelogram (transform / process)
  sampler/.style={draw, trapezium, trapezium left angle=70, trapezium right angle=110,
                  fill=orange!12, align=center, inner sep=4pt,
                  minimum width=28mm, minimum height=14mm, font=\footnotesize},
  % LLM pool: rectangle with thick border (model)
  llm/.style={draw, very thick, rounded corners=2pt, fill=purple!10,
              align=center, inner sep=4pt, minimum width=28mm,
              minimum height=14mm, font=\footnotesize},
  % validator: diamond (decision gate)
  validator/.style={draw, diamond, aspect=2, fill=red!12,
                    align=center, inner sep=2pt, font=\footnotesize,
                    minimum width=22mm},
  % output: same as corpus to convey "this is a corpus"
  outc/.style={corpus, fill=green!12},
]
  % Inputs (top of left column)
  \node[corpus]                          (s1) {Medical seeds};
  \node[corpus, below=4mm of s1]         (s2) {Finance seeds};
  \node[corpus, below=4mm of s2]         (s3) {Law seeds};

  % Axis sampler (middle)
  \node[sampler, right=of s2]            (smp) {Axis sampler\\\scriptsize QI \texttimes\ framing\\\scriptsize \texttimes\ placement \texttimes\ adv};

  % LLM pool (middle-right)
  \node[llm, right=of smp]               (pool) {LLM pool\\\scriptsize Qwen, Mistral, Phi-3\\\scriptsize {+}Yi (held-out)};

  % Validator (right of pool, gate)
  \node[validator, right=of pool]        (v)   {Validator};

  % Outputs (right of validator)
  \node[outc, right=14mm of v, yshift=10mm] (ou) {Unsafe corpus};
  \node[outc, right=14mm of v, yshift=-10mm] (ob) {Borderline-safe};

  % Arrows
  \draw[->] (s1.east) -- (smp.north west);
  \draw[->] (s2.east) -- (smp.west);
  \draw[->] (s3.east) -- (smp.south west);
  \draw[->] (smp)     -- (pool);
  \draw[->] (pool)    -- (v);
  \draw[->] (v.east)  -- (ou.west) node[midway, above, font=\scriptsize, sloped]{accept};
  \draw[->] (v.east)  -- (ob.west) node[midway, below, font=\scriptsize, sloped]{borderline};

  % Reject loop back to LLM pool
  \draw[->, dashed, gray] (v.south) .. controls +(0,-9mm) and +(0,-9mm) ..
        node[font=\scriptsize, midway, below]{reject \& retry} (pool.south);
\end{tikzpicture}%
}
\caption{Synthetic data generation pipeline. The same axis-stratified
multi-LLM pipeline is instantiated three times (medical, finance, law)
with domain-specific seed corpora, QI taxonomies
(Tab.~\ref{tab:qimap}), and validator extras. Three open-weight
generators populate the training pool; Yi-1.5-9B is held out for
cross-generator evaluation. Each generated record is rejected by the
validator if it contains direct identifiers, leaks unsanctioned
quasi-identifier patterns, or violates adversarial-mode constraints.
Borderline-safe records are produced by a separate prompt template on
the same generators (\S\ref{sec:data:borderline}).}
\label{fig:datapipeline}
\end{figure*}

% -----------------------------------------------------------------------------
% FIGURE 3 — Detection framework (§6)
% Dual one-class density estimator with discriminator and abstain region.
% -----------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
  font=\small,
  >=Stealth,
  node distance=5mm and 8mm,
  inp/.style={draw, rounded corners=2pt, fill=gray!6, align=center,
              minimum width=22mm, minimum height=7mm, inner sep=2pt},
  enc/.style={draw, rounded corners=2pt, fill=blue!8, align=center,
              minimum width=18mm, minimum height=6mm, inner sep=2pt,
              font=\scriptsize},
  fuse/.style={draw, fill=blue!18, circle, minimum size=6mm, inner sep=0pt,
               font=\scriptsize},
  det/.style={draw, rounded corners=2pt, align=center,
              minimum width=24mm, minimum height=10mm, inner sep=2pt,
              font=\scriptsize},
  thresh/.style={draw, fill=yellow!15, rounded corners=2pt, align=center,
                 minimum width=24mm, minimum height=8mm, inner sep=2pt},
  outp/.style={draw, rounded corners=2pt, align=center,
              minimum width=14mm, minimum height=6mm, inner sep=2pt,
              font=\scriptsize},
]
  \node[inp] (q) {answer text\\\textit{(Q\&A pair)}};

  \node[enc, right=of q, yshift=8mm] (e1)  {qwen3};
  \node[enc, right=of q]             (e2)  {bge-m3};
  \node[enc, right=of q, yshift=-8mm](e3)  {e5};

  \node[fuse, right=of e2] (f) {$\oplus$};

  \node[det, fill=green!10, right=14mm of f, yshift=10mm]  (ds) {T3+OCSVM$_{\text{safe}}$\\\emph{trained on safe + aug}\\$\sigma_s$};
  \node[det, fill=red!10,   right=14mm of f, yshift=-10mm] (du) {T3+OCSVM$_{\text{unsafe}}$\\\emph{trained on unsafe}\\$\sigma_u$};

  % delta sits to the right of ds/du so it never overlaps either box
  \node[fuse] (delta) at ($(ds.east)!0.5!(du.east) + (10mm,0)$) {$-$};
  \node[thresh, right=20mm of delta] (th) {threshold $\tau$\\+ abstain gate};

  \node[outp, right=14mm of th, yshift=10mm, fill=green!15] (ok)   {safe};
  \node[outp, right=14mm of th, fill=red!18]                (flag) {flag};
  \node[outp, right=14mm of th, yshift=-10mm, fill=yellow!25] (abs) {abstain};

  % arrows -- all three encoder arrows fan out from the middle of q's right edge
  \draw[->] (q.east) -- (e1.west);
  \draw[->] (q.east) -- (e2.west);
  \draw[->] (q.east) -- (e3.west);
  \draw[->] (e1) -- (f);
  \draw[->] (e2) -- (f);
  \draw[->] (e3) -- (f);
  \draw[->] (f.east) -- (ds.west);
  \draw[->] (f.east) -- (du.west);
  \draw[->] (ds.east) -- (delta.north west) node[midway, above, font=\scriptsize]{$\sigma_s$};
  \draw[->] (du.east) -- (delta.south west) node[midway, below, font=\scriptsize]{$\sigma_u$};
  \draw[->] (delta.east) -- (th.west) node[midway, above=6pt, font=\scriptsize]{$\delta = \sigma_u - \sigma_s$};
  % all three output arrows originate from th.east (centre of right edge)
  \draw[->] (th.east) -- (ok.west);
  \draw[->] (th.east) -- (flag.west);
  \draw[->] (th.east) -- (abs.west);
\end{tikzpicture}%
}
\caption{Layer-2 detector architecture. The Q\&A pair is encoded by
three frozen text encoders (qwen3, bge-m3, e5) and concatenated. Two
one-class detectors are trained in parallel: $\sigma_s$ on the safe
corpus (in v4, augmented with $4{,}000$ Mistral-generated borderline
records), and $\sigma_u$ on the unsafe corpus. The discriminator
$\delta = \sigma_u - \sigma_s$ is thresholded by $\tau$; an explicit
both-OOD gate routes points where neither distribution claims the
input to abstain (\S\ref{sec:disc:bothood}).}
\label{fig:detector}
\end{figure*}

% -----------------------------------------------------------------------------
% FIGURE 4 — Three-domain results bar chart (§8)
% pgfplots groupplot showing v3 collapse and v4 recovery on the
% borderline-safe stress test.
% -----------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\pgfplotsset{
  resbar/.style={
    ybar=2pt,
    bar width=10pt,
    width=8.5cm,
    height=5.0cm,
    enlarge x limits=0.18,
    ymajorgrids,
    grid style={dashed, gray!30},
    legend style={at={(0.02,0.98)}, anchor=north west, font=\scriptsize,
                  draw=none, fill=white, fill opacity=0.9},
    legend cell align=left,
    symbolic x coords={Medical, Finance, Law},
    xtick=data,
    xlabel={},
    every axis plot/.append style={fill opacity=0.85, draw opacity=1},
  },
}
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=2 by 1, horizontal sep=14mm},
  resbar,
]
% =====================================================================
% LEFT panel — THE DIAGNOSTIC.
% Same detector (T3+GMM-v3), two test pairings: within-distribution vs
% borderline-safe. The 16-27pp AUROC gap exposes the case-style confound.
% =====================================================================
\nextgroupplot[
  title={\small\textbf{(a) The diagnostic}: T3+GMM-v3 across two test pairings},
  ylabel={AUROC (T3+GMM-v3)},
  ymin=0.6, ymax=1.04,
  ytick={0.60, 0.70, 0.80, 0.90, 1.00},
  nodes near coords, nodes near coords style={font=\tiny,
    /pgf/number format/fixed, /pgf/number format/precision=3,
    /pgf/number format/fixed zerofill},
]
\addplot+[fill=blue!50,  draw=blue!75!black] coordinates
  {(Medical, 0.9930) (Finance, 0.9819) (Law, 0.9368)};
\addplot+[fill=red!55,   draw=red!75!black]  coordinates
  {(Medical, 0.7179) (Finance, 0.7374) (Law, 0.7756)};
\legend{within-dist, borderline}

% =====================================================================
% RIGHT panel — THE FIX.
% Same test pairing (borderline), two detector configs (v3 vs v4 at tau=0).
% The drop from 77-85% to 4-35% is the T3+OCSVM-v4 recovery.
% =====================================================================
\nextgroupplot[
  title={\small\textbf{(b) The fix}: borderline FPR @ $\tau{=}0$, v3 vs.\ v4},
  ylabel={Borderline FPR @ $\tau{=}0$ (\%)},
  ymin=0, ymax=100,
  ytick={0, 25, 50, 75, 100},
  nodes near coords, nodes near coords style={font=\tiny,
    /pgf/number format/fixed, /pgf/number format/precision=1},
]
\addplot+[fill=red!55,    draw=red!75!black]    coordinates
  {(Medical, 85.4) (Finance, 77.8) (Law, 77.5)};
\addplot+[fill=green!55,  draw=green!50!black]  coordinates
  {(Medical, 4.4) (Finance, 35.1) (Law, 4.3)};
\legend{T3+GMM-v3, T3+OCSVM-v4}
\end{groupplot}
\end{tikzpicture}%
}
\caption{\textbf{The case-style confound and its remediation.}
\textbf{(a) The diagnostic.} The same baseline detector (T3+GMM-v3),
evaluated against two different test pairings, scores AUROC
$\in [0.94, 0.99]$ on within-distribution holdout (blue) but only
$[0.72, 0.78]$ on the borderline-safe stress test (red). The gap is
the empirical signature of the case-style confound: T3+GMM-v3 has learned
referential client/patient/matter voice as a proxy for QI presence,
not QI presence itself. The two AUROC bands do not overlap, across
three independently constructed domains.
\textbf{(b) The fix.} Borderline FPR at the conservative operating
point ($\tau{=}0$) drops from $77$--$85\%$ under T3+GMM-v3 (red) to
$4.3$--$35\%$ under T3+OCSVM-v4 (green). The recipe is portable to all
three domains; finance carries an elevated residual ($35.1\%$)
attributable to quantitative content overlap on borderline subtypes
(\S\ref{sec:disc:generalization}, Tab.~\ref{tab:borderline:strata}).}
\label{fig:results}
\end{figure*}

